Performance-Portable Numerical Relativity with AthenaK

We present the numerical relativity module within AthenaK, an open source performance-portable astrophysics code designed for exascale computing applications. This module employs the Z4c formulation to solve the Einstein equations. We demonstrate its accuracy through a series of standard numerical relativity tests, including convergence of the gravitational waveform from binary black hole coalescence. Furthermore, we conduct scaling tests on OLCF Frontier and NERSC Perlmutter, where AthenaK exhibits excellent weak scaling efficiency of 80% on up to 65,536 AMD MI250X GPUs on Frontier (relative to 4 GPUs) and strong scaling efficiencies of 84% and 77% on AMD MI250X and NVIDIA A100 GPUs on Frontier and Perlmutter respectively. Additionally, we observe a significant performance boost, with two orders of magnitude speedup ($\gtrsim 200\times$) on a GPU compared to a single CPU core, affirming that AthenaK is well-suited for exascale computing, thereby expanding the potential for breakthroughs in numerical relativity research.

==> tables/single-core_performance.tex <==
\begin{deluxetable*}{lcccccc}
%\tabletypesize{\footnotesize}
\tabletypesize{\footnotesize}
\tablecolumns{6} \tablewidth{30pt}
\tablecaption{Single device performance of \ak{}\label{table:single-perf}}
\setlength{\tabcolsep}{+0.05cm}
\tablehead{
\colhead{\begin{tabular}{l} {} \\ \end{tabular}} &
\colhead{\begin{tabular}{c} CPU node\\ (\app{})  \end{tabular}} &
\colhead{\begin{tabular}{c} CPU node\\ (\ak{})   \end{tabular}} &
\colhead{\begin{tabular}{c} Nvidia\\V100   \end{tabular}} &
\colhead{\begin{tabular}{c} Nvidia\\A100   \end{tabular}} &
\colhead{\begin{tabular}{c} AMD\\ MI250  \end{tabular}} &
}
\startdata
%
Non-relativistic hydro    &50  &9.83  &2.66& 12.49 & 2.50 \\ 
Non-relativistic MHD    &25  &18.76&3.38&22.14 & 2.5 \\
\hline
Special relativistic hydro    &25 & 18.76 & 3.38 & 22.14 & 2.5  \\
Special relativistic MHD    &25  & 18.76 & 3.38 & 22.14 & 2.5  \\
\hline
General relativistic hydro          &25 & 18.76 & 3.38 &  22.14 & 2.5 \\
General relativistic MHD              &25  & 18.76 & 3.38 & 22.14 & 2.5 \\
General relativistic radiation MHD   & 2.2 & 18.76 & 3.38 & 22.14 & 2.5 \\
\enddata
\tablenotetext{(a)}{~Add notes here.} 
\end{deluxetable*}


